VisualLens: Personalization through Task-Agnostic Visual History

Existing recommendation systems either rely on user interaction logs, such as online shopping history for shopping recommendations, or focus on text signals. However, item-based histories are not always accessible, and are not generalizable for multimodal recommendation. We hypothesize that a user's visual history -- comprising images from daily life -- can offer rich, task-agnostic insights into their interests and preferences, and thus be leveraged for effective personalization. To this end, we propose VisualLens, a novel framework that leverages multimodal large language models (MLLMs) to enable personalization using task-agnostic visual history. VisualLens extracts, filters, and refines a spectrum user profile from the visual history to support personalized recommendation. We created two new benchmarks, Google-Review-V and Yelp-V, with task-agnostic visual histories, and show that VisualLens improves over state-of-the-art item-based multimodal recommendations by 5-10% on Hit@3, and outperforms GPT-4o by 2-5%. Further analysis shows that VisualLens is robust across varying history lengths and excels at adapting to both longer histories and unseen content categories.

==> personal_commands.tex <==
\usepackage{pifont}% http://ctan.org/pkg/pifont
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\newcommand{\bill}[1]{\textcolor{blue}{#1$_{BZ}$}}

% ourmethod
\newcommand{\ourmethod}{\textsc{VisualLens}\xspace}
% \newcommand{\ourmethodhighlight}{\textbf{M}ixed \textbf{E}xtracted \textbf{R}epresentation with \textbf{I}terative refinement and joint \textbf{T}raining\xspace}
\newcommand{\ourmethodshort}{\textsc{VisualLens}\xspace}

% dataset
\newcommand{\googledatafull}{Google Review-Vision\xspace}
\newcommand{\yelpdatafull}{Yelp-Vision\xspace}
\newcommand{\googledata}{Google Review-V\xspace}
\newcommand{\yelpdata}{Yelp-V\xspace}

% method
\newcommand{\unimp}{UniMP\xspace}

% models
\newcommand{\llama}{Llama-3.1\xspace}
\newcommand{\gpto}{GPT-4o\xspace}
\newcommand{\paligemma}{PaliGemma\xspace}
\newcommand{\minicpm}{MiniCPM-V2.5\xspace}
\newcommand{\llava}{LLaVA-v1.6\xspace}
\newcommand{\clip}{CLIP ViT-L/14@336px\xspace}

\newcommand{\todo}{X\xspace}

\RequirePackage{xcolor}
\definecolor{metablue}{HTML}{0064E0}
\definecolor{metafg}{HTML}{1C2B33}
\definecolor{metabg}{HTML}{F1F4F7}

\usepackage{array}
\newcommand{\PreserveBackslash}[1]{\let\temp=\\#1\let\\=\temp}
\newcolumntype{C}[1]{>{\PreserveBackslash\centering}p{#1}}
\newcolumntype{R}[1]{>{\PreserveBackslash\raggedleft}p{#1}}
\newcolumntype{L}[1]{>{\PreserveBackslash\raggedright}p{#1}}

\newcommand{\kkDL}{{\color{purple} kkDL}\xspace}
\newcommand{\kqo}{{\color{brown} k4qo}\xspace}
\newcommand{\Tfca}{{\color{blue} Tfca}\xspace}

==> table/dataset_stats.tex <==
\begin{table}[t]
    \centering
    \tabcolsep 2pt
    \resizebox{\linewidth}{!}{
    \begin{NiceTabular}{p{15mm}p{12mm}p{10mm}p{10mm}p{15mm}p{10mm}p{10mm}p{10mm}}
    \CodeBefore
    % \rectanglecolor{metabg}{3-4}{4-4}
    % \rectanglecolor{metabg}{7-8}{7-9}
    % \rectanglecolor{metabg}{8-9}{7-9}
    \Body
    \toprule
    Dataset name & Train split & Dev split & Test split & Categories & Avg. \# images & Avg. \# GT & Avg. \# cand. \\
    \midrule
    GR-V & 15.69M & 2K & 200K & 66 & 157.0 & 2.7 & 43.1 \\ 
    Yelp-V & 4.12M & 2K & 100K & 35 & 263.6 & 8.2 & 66.7  \\
    \bottomrule
    \end{NiceTabular}
    }
    \caption{Dataset statistics of Google Review-Vision (GR-V) and Yelp-Vision (Yelp-V).}
    \label{table:dataset_stats}
\end{table}
